Evaluating Test-Time Scaling of General LLM Agents

LLM agents are increasingly expected to operate as general-purpose systems that resolve real-world user requests, yet their dynamic scaling behavior in realistic environments remains poorly understood. In this paper, we systematically investigate two principal test-time scaling axes of LLM agents: sequential scaling through extended interaction and parallel scaling through trajectory sampling. We first introduce a realistic benchmark that provides one unified framework for evaluating LLM agents across search, coding, reasoning, and tool-use domains, more faithfully reflecting the heterogeneity of real-world deployments. Evaluating ten leading LLM agents reveals substantial performance degradation when transitioning from domain-specific evaluations to this realistic setting. Building on this foundation, we progressively scale test-time compute along fine-grained increments to characterize the performance upper bound. We find that neither scaling axis can consistently yield meaningful gains from additional test-time compute in realistic environments, a phenomenon we attribute to two fundamental limitations: the scaling plateau that bottlenecks sequential scaling and the verification gap that undermines parallel scaling. Code is publicly available at https://github.com/cxcscmu/General-AgentBench.

==> src/4tts_analysis.tex <==


\section{Dynamic behavior of Test-Time Scaling}

% In this section, we present a systematic study of test-time scaling behavior under the omni agentic setting. Our goal is to characterize how general-agent performance evolves with increased test-time computation, and to examine whether performance gains from test-time scaling translate into improvements in real-world agentic interactions.

In this section, we present a systematic study of test-time scaling behavior of general LLM agents. Section~\ref{4.1} introduces the scaling strategies, with results and findings presented in Sections~\ref{4.2} and~\ref{4.3}.


\subsection{Scaling Methodology}\label{4.1}

We investigate test-time scaling through two complementary paradigms: \textbf{Parallel Scaling} and \textbf{Sequential Scaling}, which correspond to distinct axes of computational allocation—breadth of exploration versus depth of exploitation. Compared with more sophisticated test-time scaling techniques such as self-correction~\citep{Madaan2023SelfRefine}, beam search~\citep{Yao2023ToT}, or MCTS~\citep{Zhou2023LATS}, these two strategies are the most commonly adopted and easiest to deploy in real-world agentic systems.

\paragraph{Parallel Scaling.}
In the parallel scaling regime, we independently sample $K$ trajectories for each query. Increasing $K$ expands the reachable action space, thereby increasing the likelihood that the agent explores at least one trajectory containing a correct solution, relative to the single-shot baseline ($K=1$). 

However, in the absence of external oracles or human feedback—particularly in real-world deployments—parallel scaling alone is insufficient: agents must also be capable of evaluating and selecting the best outcome from their own generated trajectories. To assess this ability, we introduce this \textbf{Self-Choice} setting, in which the agent evaluates its parallelly sampled outputs using one of the following strategies:

\textbf{(1) Point-wise choice.}  
The agent independently evaluates each sampled trajectory and assigns a binary judgment. Performance is measured by the alignment between the model’s judgments and oracle labels, averaged over trajectories that are correct under oracle evaluation.

\textbf{(2) Pair-wise choice.}  
The agent compares two sampled trajectories at a time and iteratively promotes the superior one through a bubble-sort-style selection process. After $K-1$ pairwise comparisons, a single trajectory is selected as the final output, and performance is evaluated based on the correctness of this selected trajectory.

Overall, self-choice reflects the practical effectiveness of parallel scaling, while past@$K$ serves as an upper bound that reveals the solution potential.

\paragraph{Sequential Scaling.}
In contrast, sequential scaling increases computational depth by extending the interaction horizon. As the agent engages with the environment, the conversation context progressively grows. When the agent attempts to terminate an episode (e.g., by emitting an End-of-Turn token), we inject an additional round of environment feedback to encourage further reflection on prior reasoning and exploration of alternative solution paths.

To quantify scaling behaviors under both paradigms, we plot task accuracy against the number of independent samples ($K$) for parallel scaling, and against cumulative context length for sequential scaling in Figure~\ref{fig:tts}. Due to the cost of API-based inference, each model is sampled at most four times, and context length is scaled up to 196K tokens. A detailed cost analysis for reproducibility is provided in the Appendix~\ref{appendix:cost}.

\subsection{Sequential Scaling}\label{4.2}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/search_heatmap_159_168.pdf}
\caption{\textbf{Instance-level correctness dynamics under sequential scaling.}
We randomly sample 10 instances from the reasoning domain and track their correctness across increasing context lengths. Red indicates incorrect predictions and blue indicates correct ones. Most instances exhibit stagnant or oscillatory behavior, repeating prior successes while failing on unresolved cases, with some fluctuating between correct and incorrect across steps.}
    \label{fig:per_instance}
\end{figure}

Sequential scaling exhibits behavior that departs markedly from our expectations, shown in the bottom of Figure~\ref{fig:tts}. Although several models on certain benchmarks show performance improvements, such as Qwen3-235B on the Search domain and Deepseek-v3.2 on the Reason domain, most show little to no consistent improvement despite allocating additional computational resources through iterative reasoning and reflection. 

We categorize sequential scaling behaviors into two distinct regimes. (1) \textbf{Stagnant fluctuation}: In domains such as reasoning, performance oscillates within a narrow range despite increased computation. This pattern suggests a limited capacity for agents to explore novel solution paths within extended interaction traces, coupled with a diminished ability to maintain coherence—likely due to the agent's finite context processing capacity. (2) \textbf{Saturation and degradation}: In coding domains, models initially benefit from additional reasoning steps; however, beyond an important scaling plateau, performance consistently deteriorates and fails to recover. Figure~\ref{fig:per_instance} shows how instance-level correctness for several data entries changes as the context length increases. We observe that agents either repeatedly succeed on queries they already handle well while failing to progress on unsuccessful cases, or exhibit unstable behavior with accuracy fluctuating between 0 and 1 across interaction steps. These observations further validate our summarization regarding the inherent limitations of sequential scaling.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/context_scaling_regions.pdf}
        \caption{Sequential scaling behavior of Gemini~2.5-Flash and Qwen3-235B across domains, with inherent context lengths indicated by the dashed line. Performance scales positively as interaction history approaches and slightly exceeds the inherent context; however, it saturates or degrades once the context extends significantly beyond this threshold. This limit represents the ``scaling plateau" of sequential scaling, beyond which further history yields diminishing returns.}
    \label{fig:inherent_context}
\end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/agentic_scaling_pairwise_facet.pdf}
    \caption{\textbf{Verification gap between generation and self-choice.}
Across four domains, we observe a consistent gap between solution generation and verification: as the number of samples increases, correct solutions appear more frequently in the sampled set, yet models often fail to identify and select them. The dashed and dotted curves represent two self-choice strategies, while the diamond denotes a stronger evaluator, GPT-5.}
    \label{fig:self-choice}
\end{figure*}

To better understand how this scaling plateau occurs, we analyze performance relative to an agent’s inherent context length—defined as the total context naturally accumulated when completing a task without artificial constraints on interaction depth. By integrating data from Qwen3-235B and Gemini 2.5-Flash (as seen in Figure~\ref{fig:tts}) with new experimental results on smaller context windows, we observed a distinct performance ceiling. As shown in Figure~\ref{fig:inherent_context}, both models exhibit an initial upward trend, approaching peak performance as they reach their inherent context limits. However, once the accumulated context passes a specific threshold ( for example, approximately 112K for Qwen3-235B and 96K for Gemini 2.5-Flash in the search domain), performance typically plateaus or begins to degrade. In these instances, additional computation and time yield no further gains. This suggests the existence of a ``\textbf{scaling plateau}": a maximum effective context length under sequential scaling, beyond which raw interaction history offers diminishing or zero practical returns. Notably, this ceiling varies across domains, reflecting the unique demands each task places on context utilization and computational efficiency.

Taken together, these results indicate that simply allocating more computation by extending raw interaction histories rarely leads to meaningful performance gains, contradicting previous observations in non-agentic settings~\citep{muennighoff2025s1}. Long-horizon agentic tasks expose fundamental challenges in context utilization and reasoning stability, highlighting the need for more effective mechanisms for context management and reasoning control under sequential scaling~\citep{zhang2025agentic, claudecontexxt}.

\subsection{Parallel Scaling}\label{4.3}

We observe a monotonic increase in \textbf{pass@K} as the number of sampled trajectories grows (Figure~\ref{fig:tts}, top). Increasing $K$ from 1 to 4 yields an average improvement of roughly 50\%, with DeepSeek-V3.2 exhibiting the largest gains—approaching a twofold improvement in both coding and reasoning domains.

However, pass@K only reflects an idealized upper bound. In practice, the effectiveness of parallel scaling depends on an agent’s ability to evaluate and select among its own sampled trajectories, which is captured by self-choice performance. As shown by the gap between the solid lines (pass@K) and the dashed or dotted lines (self-choice) in Figure~\ref{fig:self-choice}, self-choice performance consistently lags behind the pass@K upper bound regardless of the strategy. In some cases, self-choice performance even degrades as $K$ increases. While the coding domain exhibits the smallest gap between pass@K and self-choice, in most settings self-choice gains saturate quickly and fail to track the continued improvement of pass@K.

To examine whether this gap stems from limited verifier capability, we replace the model’s internal self-judgment with an external verifier, GPT-5, and perform point-wise evaluation of sampled trajectories from all models. As shown by the diamond line in Figure~\ref{fig:self-choice}, GPT-5 generally underperforms models’ own self-judgment. Notably, even at $K=1$, GPT-5 occasionally misclassifies correct trajectories as incorrect, introducing a non-trivial gap between pass@1 and GPT-5–based verification. We hypothesize that this effect arises from \textbf{solution familiarity}: models are better at evaluating their own generations, which align closely with their internal reasoning patterns, whereas external verifiers may struggle to accurately assess unfamiliar execution traces.

Overall, these results reveal a fundamental gap between models’ generation capacity and their ability to reliably select correct solutions, which ultimately limits the practical utility of parallel scaling. 

% Bridging this gap requires improving agents’ self-evaluation robustness and reliability, rather than solely expanding the generation space.




% \cx{I think it is clear that now we should treat the pairwise choice as the parallel scaling, as it is the actual scaling method, then the pass at K is the upper bound to show the verification gap... hopefully we have all the results to change the plots, and the writing changes can be done in the next pass. Right now the oracle pass at K upper bound is mixed with the actual sequence scaling, making it quite confusing}\xiaochuan{check}

% \cx{then you can move the pairwise self choice descriptions as part of the previou subsection as scaling methods (and it is realy a scaling method now)}\xiaochuan{check}



% \cx{will be great if we can show the inherit reasoning context length of at least one model's distributions on all the testing user requests, to show this important message, likely here in this paper...}\xiaochuan{check}



==> src/5_analysis_main.tex <==
\section{Attention Analysis}\label{section5}

\subsection{Comparison between Linear and Full Attention}

Across both parallel and sequential test-time scaling, Qwen3-Next shows weaker performance gains than full-attention models. To investigate this gap, we analyze the impact of its hybrid attention design. We compare it with Qwen3-235B-A22B, a full-attention baseline, by measuring average attention distance in the final reasoning step. Specifically, for every full-attention head, we record the top-$k$ attended tokens and compute their token-distance relative to the beginning of the final output span. For Gated DeltaNet, which does not explicitly expose standard attention weights, we adopt a mathematically equivalent procedure to recover the effective top-$k$ contributing tokens and compute the corresponding distances (details provided in Appendix~X).

Figure~\ref{fig:attention_analysis} visualizes the resulting heatmaps. We find that full attention consistently exhibits larger average attention distances than Gated DeltaNet. This is evident both in the comparison between Qwen3-235B and Qwen3-Next, as well as within Qwen3-Next itself when contrasting its Gated Attention and DeltaNet components. These results indicate that full attention is more effective at capturing long-range dependencies, which likely contributes to its superior scaling consistency under long-context agentic settings


% \cx{all sec 5 are interesting, but too verbose, can be much more concise and reduce the space into half? I really want to inherit reasoning token budget study as it illustates a new and clear picture of what seq scaling does not beyond certain token lens. then if we have space we can move some case studies to main paper}\xiaochuan{check. Shortened the three subsections.}

\begin{figure}[t]
    \centering

    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/attention_mean_distance_qwen3_235b.pdf}
        \caption{Qwen3-235B (full attention)}
        \label{fig:attn_qwen3_235b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/attention_mean_distance_qwen3_next.pdf}
        \caption{Qwen3-Next (hybrid attention)}
        \label{fig:attn_qwen3_next}
    \end{subfigure}

    \caption{\textbf{Mean top-$k$ attention distance across layers and heads.}
    We report the average distance between the top-$k$ attended tokens and the beginning of the model’s final output span.
    \textbf{Left}: Qwen3-235B with full attention.
    \textbf{Right}: Qwen3-Next with hybrid Gated Attention and Gated DeltaNet.}
    \label{fig:attention_analysis}
\end{figure}

==> src/apppendix_attention.tex <==
\section{Full Attention: Softmax Attention}

\subsection{Standard Attention Computation}
For Full Attention layers, we utilize Scaled Dot-Product Attention:
\begin{equation}
\text{Attention}(Q, K, V) = \text{softmax}\left(\frac{QK^T}{\sqrt{d_k}}\right) V
\end{equation}

\subsection{Qwen3-Next Full Attention Features}
The implementation includes specific architectural enhancements:
\begin{enumerate}
    \item \textbf{Gated Projection}: The hidden state $h$ is projected to generate both the queries and a gating signal:
    \begin{equation}
    [Q, G] = \text{split}(W_{qg} \cdot h)
    \end{equation}
    
    \item \textbf{Normalization}: RMSNorm is applied to $Q$ and $K$ to stabilize training:
    \begin{equation}
    Q_{norm} = \text{RMSNorm}(Q), \quad K_{norm} = \text{RMSNorm}(K)
    \end{equation}
    
    \item \textbf{Rotary Position Embedding (RoPE)}:
    \begin{equation}
    Q', K' = \text{RoPE}(Q_{norm}, K_{norm}, \text{pos})
    \end{equation}
    
    \item \textbf{Gated Output}: The final attention result is modulated by the sigmoid-activated gate:
    \begin{equation}
    \text{output} = \sigma(G) \odot \text{Attention}(Q', K', V)
    \end{equation}
\end{enumerate}

\section{Linear Attention: Gated Delta Rule}

\subsection{DeltaNet Mechanism}
The Gated Delta Rule maintains a key-value memory state $S_t$. Unlike standard linear attention, it utilizes a "Delta" update to minimize prediction error.

\subsubsection{State Update Formulas}
For each time step $t$, the state $S \in \mathbb{R}^{d_k \times d_v}$ is updated as follows:
\begin{enumerate}
    \item \textbf{State Decay}: $\tilde{S}_{t-1} = \gamma_t \cdot S_{t-1}$, where $\gamma_t = \exp(g_t)$.
    \item \textbf{Prediction Error}: $\delta_t = v_t - \tilde{S}_{t-1} k_t$.
    \item \textbf{Delta Rule Update}:
    \begin{equation}
    S_t = \gamma_t S_{t-1} + \beta_t (k_t \otimes \delta_t)
    \end{equation}
    where $\beta_t \in [0, 1]$ acts as a dynamic learning rate.
\end{enumerate}

\subsection{Converting DeltaNet to Q, K, V Form}

\subsubsection{Effective Keys Concept}
To extract an $N \times N$ matrix from a recurrent process, we track \textbf{effective keys} $\hat{k}_j^{(i)}$, representing the contribution of position $j$ to the state at time $i$.

Update rules for position $i$:
\begin{align}
\hat{k}_j^{(i)} &= \gamma_i \hat{k}_j^{(i-1)} - \beta_i (k_i \cdot (\gamma_i \hat{k}_j^{(i-1)})) k_i, \quad \forall j < i \\
\hat{k}_i^{(i)} &= \beta_i k_i
\end{align}

\subsubsection{Attention Weight Extraction}
The simulated attention weights are computed as:
\begin{equation}
\boxed{A_{ij} = q_i \cdot \hat{k}_j^{(i)}}
\end{equation}

\subsection{Decay Matrix}
The cumulative decay $D_{ij}$ between positions $j$ and $i$ ($j \leq i$) is:
\begin{equation}
D_{ij} = \exp \left( \sum_{t=j+1}^{i} g_t \right)
\end{equation}

\subsection{Complete Extraction Algorithm}

\begin{algorithm}[H]
\caption{Gated Delta Rule Attention Matrix Extraction}
\begin{algorithmic}[1]
\Require $Q, K, V \in \mathbb{R}^{n \times d}$, decay gate $g \in \mathbb{R}^n$, learning rate $\beta \in \mathbb{R}^n$
\Ensure Attention matrix $A \in \mathbb{R}^{n \times n}$
\State $Q, K \gets \text{L2Norm}(Q), \text{L2Norm}(K)$
\State $S \gets \mathbf{0}^{d_k \times d_v}$
\State $\hat{K} \gets \mathbf{0}^{n \times d_k}$ \Comment{Matrix of effective keys}
\For{$i = 1$ to $n$}
    \State $\gamma_i \gets \exp(g_i)$
    \State $\hat{K}_{1:i-1} \gets \gamma_i \hat{K}_{1:i-1} - \beta_i (\hat{K}_{1:i-1} k_i) \otimes k_i$ \Comment{Parallel unlearning update}
    \State $\hat{K}_i \gets \beta_i k_i$
    \State $A_{i, 1:i} \gets q_i \hat{K}_{1:i}^T$
\EndFor
\State \Return $A$
\end{algorithmic}
\end{algorithm}

\section{Unique Properties and Metrics}

\subsection{Weight Interpretation}
\begin{itemize}
    \item \textcolor{blue}{\textbf{Positive Weights ($A_{ij} > 0$)}}: Information retrieval/reinforcement.
    \item \textcolor{red}{\textbf{Negative Weights ($A_{ij} < 0$)}}: Error correction/interference cancellation.
\end{itemize}

\subsection{Analysis Metrics}
\begin{enumerate}
    \item \textbf{Positive/Negative Mass}: $M^+ = \sum A_{ij}^+, \quad M^- = \sum |A_{ij}^-|$.
    \item \textbf{Effective Context Length}:
    \begin{equation}
    L_{\text{eff}} = \frac{\sum_{j=1}^{i} D_{ij} \cdot (i - j + 1)}{\sum_{j=1}^{i} D_{ij}}
    \end{equation}
\end{enumerate}

\section{Summary Comparison}

\begin{table}[h]
\centering
\begin{tabular}{lll}
\toprule
\textbf{Feature} & \textbf{Full Attention} & \textbf{Linear Attention (Delta)} \\
\midrule
Weight Range & $[0, 1]$ & $(-\infty, +\infty)$ \\
Normalization & RMSNorm + Softmax & L2Norm \\
Positional Encoding & RoPE & Decay Gate $\gamma_t$ \\
Memory Complexity & $O(N^2)$ & $O(N)$ (Recurrent Form) \\
\bottomrule
\end{tabular}
\caption{Comparison of Attention Mechanisms in Qwen3-Next}
\end{table}

==> tables/analysis_2_scaling_consistency.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Outcome transition patterns across domains under sequential scaling.
We compare point-wise correctness between the initial (short) context and the maximum context length
for \textsc{Gemini-2.5-Flash} and \textsc{Qwen3-Next}.}
\label{tab:outcome_transition}
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l cc cc cc cc}
\toprule
\textbf{Transition Type}
& \multicolumn{2}{c}{\textbf{Search}}
& \multicolumn{2}{c}{\textbf{Code}}
& \multicolumn{2}{c}{\textbf{Reason}}
& \multicolumn{2}{c}{\textbf{Tool-Use}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& \rotatebox{90}{\textbf{Gemini}}
& \rotatebox{90}{\textbf{Qwen3}}
& \rotatebox{90}{\textbf{Gemini}}
& \rotatebox{90}{\textbf{Qwen3}}
& \rotatebox{90}{\textbf{Gemini}}
& \rotatebox{90}{\textbf{Qwen3}}
& \rotatebox{90}{\textbf{Gemini}}
& \rotatebox{90}{\textbf{Qwen3}} \\
\midrule
\emph{Failure} to \emph{Correct}
& 6   & 2   & 6   &     & 6   & 1   & 4   & 4   \\
\emph{Correct} to \emph{Failure}
& 2   & 9   & 2   &     & 6   & 3   & 2   & 4   \\

\cdashline{1-9}

Consistent \emph{Correct}
& 29  & 21  & 29  &     & 31  & 34  & 4   & 20  \\
Consistent \emph{Failure}
& 162 & 167 & 162 &     & 32  & 37  & 40  & 22   \\
\bottomrule
\end{tabular}
\end{table}


==> tables/compare_previous_long_context.tex <==
\sisetup{round-mode=figures, round-precision=3}

\begin{table*}[ht]
\centering
\small
\caption{Main Results: Performance comparison across long-context and agentic benchmarks. \textbf{Agentic LongBench} highlights the performance gap between traditional retrieval-based tasks and multi-turn agentic reasoning. Bold indicates the best performance in each column. \cx{expand our tasks in each category, do not just show average.}}
% \caption{Main Results: Performance comparison across long-context and agentic benchmarks. \textbf{Agentic LongBench} highlights the performance gap between traditional retrieval-based tasks and multi-turn agentic reasoning. Bold indicates the best performance in each column.}
\label{tab:main_results}
\setlength{\tabcolsep}{8pt}
\begin{tabular}{@{} l *{3}{S[table-format=2.1]} *{5}{S[table-format=2.1]} @{}}
\toprule
\multirow{2.5}{*}{\textbf{Models}} & {\multirow{2.5}{*}{\textbf{LongB.}}} & {\multirow{2.5}{*}{\textbf{HELMET}}} & {\multirow{2.5}{*}{\textbf{MRCR}}} & \multicolumn{5}{c}{\textbf{Agentic LongBench (Ours)}} \\
\cmidrule(l){5-9} 
 & & & & {\textbf{Search}} & {\textbf{Code}} & {\textbf{Reason}} & {\textbf{Tool}} & {\textbf{All}} \\
\midrule
GPT-OSS-120B         & 47.8 & 12.9 & 32.8 & 17.6 & 16.9 & 46.7 & 65.2 & 36.6 \\
Qwen3-235B-A22B      & 58.3 & 40.8 & 40.6 & 21.7 & 36.2 & 45.3 & 62.6 & 41.5 \\
Qwen3-Next           & 53.1 & 26.3 & 27.9 & 16.1 & 22.3 & 44.0 & 55.8 & 34.6 \\
DeepSeek-V3.2        & 50.3 & 48.0 & 33.2 & 24.6 & 32.3 & 17.3 & 61.9 & 34.0 \\
DeepSeek-R1          & 58.3 & 36.9 & 39.2 & 16.6 & 23.1 & 37.3 & 44.7 & 30.4 \\
\addlinespace[0.5em] % Visual separation for Frontier models
Gemini 2.5-Flash     & 62.1 & 27.8 & 67.4 & 21.1 & 30.0 & 60.0 & 66.0 & 44.3 \\
Gemini 2.5-Pro       & 63.3 & \bfseries 63.1 & \bfseries 80.0 & 23.4 & 26.9 & 61.3 & 66.0 & 44.4 \\
Claude Haiku 4.5     & 55.3 & 50.4 & 33.3 & 23.6 & 41.5 & 54.7 & 64.5 & 36.7 \\
Claude Sonnet 4.5    & 61.8 & 49.2 & 35.5 & 26.1 & \bfseries 49.2 & 32.0 & 73.0 & 45.1 \\
GPT-5                & \bfseries 64.6 & 51.6 & 79.1 & \bfseries 55.8 & 45.4 & \bfseries 64.0 & \bfseries 78.3 & \bfseries 60.9 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/cross-domain.tex <==
\begin{table}[t]
\centering
\small
\caption{Failure analysis under the omni setting. We categorize incorrect outcomes based on whether the agent fails after invoking tools from an incorrect domain or fails despite selecting tools from the correct domain. Results are aggregated by task domain.}
\label{tab:tool_failure_recovery}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lcc}
\toprule
\textbf{Domain}
& \textbf{Failure with Incorrect-Domain Tools}
& \textbf{Failure with Correct-Domain Tools} \\
\midrule
Search    & 17 & 90 \\
Code      & 6  & 60 \\
Reason    & 2  & 46 \\
Tool-Use  & 15 & 67 \\
\midrule
Avg       & 40 (9.1\%) & 263 (60.0\%) \\
\bottomrule
\end{tabular}

\end{table}

==> tables/omni_only_main_results.tex <==
\begin{table*}[t]
\centering
\small
\caption{Main results on \textbf{General AgentBench}. Benchmarks are grouped by domain. \textbf{Avg.} denotes the mean score across all available benchmarks for each model. Bold indicates the best score.}
\label{tab:omni_only_domain_avg}
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{} l rr rr r rr r @{}}
\toprule
\multirow{2}{*}{\textbf{Models}} &
\multicolumn{2}{c}{\textbf{Search}} &
\multicolumn{2}{c}{\textbf{Code}} &
\textbf{Reason} &
\multicolumn{2}{c}{\textbf{Tool-use}} &
\multirow{2}{*}{\textbf{Avg.}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6} \cmidrule(lr){7-8}
& \textbf{BrowseComp} & \textbf{WebVoyager}
& \textbf{SWE-Bench} & \textbf{Terminal-Bench}
& \textbf{MathHay}
& \textbf{Tau2-Bench} & \textbf{MCP-Bench}
& \\
\midrule

\textit{Open-Source} \\

GPT-OSS-120B
& 4.0 & 27.7 & 12.0 & 6.3 & 38.7 & 26.0 & 63.3 & 25.4 \\

Qwen3-235B-A22B
& 8.9 & 30.8 & 20.4 & 23.8 & 32.0 & 38.3 & 66.1 & 31.5\\

Qwen3-Next
& 10.5 & 35.4 & 18.0 & 8.8 & 42.0 & 48.9 & 64.6 & 32.6 \\

DeepSeek-V3.2
& 19.4 & 46.2 & 31.8 & 22.2  & 33.3 &  \bfseries
 54.0 &  66.0 & 39.0 \\

DeepSeek-R1
& 9.7 & 43.1 & 14.0 & 8.8 & 46.7 & 17.1 & 62.2 & 28.8 \\

\hline
% \addlinespace[0.5em]
\textit{Proprietary} \\

Gemini 2.5-Flash
& 6.5 & 32.3 & 14.0 & 20.0 & 36.0 & 38.3 & 66.6 & 30.5 \\

Gemini 2.5-Pro
& 8.9 & 46.2 & 26.0 & 27.5 & 24.0 & 46.0 & 67.2 & 35.1 \\

Claude Haiku 4.5
& 17.7 & 47.7 & \bfseries
 56.0 & 25.0 & 34.7 & 44.0 & 69.0 & 42.0 \\

Claude Sonnet 4.5
& 23.1 & 56.9 & 54.0 & \bfseries
 45.0 & 36.0 & 48.0 & \bfseries
 72.9 & \bfseries 48.0 \\

GPT-5
& \bfseries
 27.4 & \bfseries
 61.5 & 36.0 & 41.3 & \bfseries
 64.0 & 32.0 & 59.1 & 45.9 \\

\bottomrule
\end{tabular}
\end{table*}


==> tables/omni_parallel_scaling.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{Pass@k results across domains under the Omni-agent setting.}
\label{tab:omni_passk_all}
\begin{tabular}{l *{2}{c c c c c}}
\toprule
\multirow{2}{*}{\textbf{Omni (Model)}} 
& \multicolumn{5}{c}{\textbf{Search}} 
& \multicolumn{5}{c}{\textbf{Code}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
& \textbf{pass@1} & \textbf{pass@2} & \textbf{pass@3} & \textbf{pass@4} & \textbf{pass@8}
& \textbf{pass@1} & \textbf{pass@2} & \textbf{pass@3} & \textbf{pass@4} & \textbf{pass@8} \\
\midrule
Qwen3-Next        & 0.1859 & 0.2462 & 0.2814 & 0.3116 & -- 
                  & -- & -- & -- & -- & -- \\
Qwen3-235B        & 0.1558 & 0.2111 & 0.2362 & 0.2663 & -- 
                  & -- & -- & -- & -- & -- \\
DeepSeek-V3.2     & running & running & running & running & running 
                  & -- & -- & -- & -- & -- \\
DeepSeek-R1-0528  & -- & -- & -- & -- & -- 
                  & -- & -- & -- & -- & -- \\
Gemini-2.5 Flash  & 0.1457 & 0.1658 & 0.2010 & 0.2261 & -- 
                  & -- & -- & -- & -- & -- \\
\midrule
\addlinespace[4pt]

\multirow{2}{*}{\textbf{Omni (Model)}} 
& \multicolumn{5}{c}{\textbf{Reason}} 
& \multicolumn{5}{c}{\textbf{Tool-use}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
& \textbf{pass@1} & \textbf{pass@2} & \textbf{pass@3} & \textbf{pass@4} & \textbf{pass@8}
& \textbf{pass@1} & \textbf{pass@2} & \textbf{pass@3} & \textbf{pass@4} & \textbf{pass@8} \\
\midrule
Qwen3-Next        & -- & -- & -- & -- & -- 
                  & -- & -- & -- & -- & -- \\
Qwen3-235B        & -- & -- & -- & -- & -- 
                  & -- & -- & -- & -- & -- \\
DeepSeek-V3.2     & -- & -- & -- & -- & -- 
                  & -- & -- & -- & -- & -- \\
DeepSeek-R1-0528  & -- & -- & -- & -- & -- 
                  & -- & -- & -- & -- & -- \\
Gemini-2.5 Flash  & -- & -- & -- & -- & -- 
                  & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/omni_parallel_selfchoice.tex <==
% Requires: \usepackage{booktabs} \usepackage{multirow} \usepackage{graphicx}
% If you want nicer spacing: \usepackage{array}

\begin{table*}[t]
\centering
\small
\scalebox{0.9}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l *{2}{c c c c c c c}}
\toprule
\multirow{3}{*}{\textbf{Omni (Model)}} 
& \multicolumn{7}{c}{\textbf{Search}} 
& \multicolumn{7}{c}{\textbf{Code}} \\
\cmidrule(lr){2-8}\cmidrule(lr){9-15}
& \multicolumn{5}{c}{\textbf{Pass@k}} & \multicolumn{2}{c}{\textbf{Self-choice}} 
& \multicolumn{5}{c}{\textbf{Pass@k}} & \multicolumn{2}{c}{\textbf{Self-choice}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-8}\cmidrule(lr){9-13}\cmidrule(lr){14-15}
& \textbf{p@1} & \textbf{p@2} & \textbf{p@3} & \textbf{p@4} & \textbf{p@8} & \textbf{point-wise} & \textbf{pair-wise}
& \textbf{p@1} & \textbf{p@2} & \textbf{p@3} & \textbf{p@4} & \textbf{p@8} & \textbf{point-wise} & \textbf{pair-wise} \\
\midrule
Qwen3-Next        & 0.1859 & 0.2462 & 0.2814 & 0.3116 & -- & 0.1156 & --  & -- & -- & -- & -- & -- & -- & -- \\
Qwen3-235B        & 0.1558 & 0.2111 & 0.2362 & 0.2663 & -- & -- & --  & -- & -- & -- & -- & -- & -- & -- \\
DeepSeek-V3.2     & -- & -- & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- & -- & -- \\
DeepSeek-R1-0528  & -- & -- & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- & -- & -- \\
Gemini-2.5 Flash  & 0.1457 & 0.1658 & 0.2010 & 0.2261 & -- & 0.1457 & 0.191  & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\addlinespace[4pt]

\multirow{3}{*}{\textbf{Omni (Model)}} 
& \multicolumn{7}{c}{\textbf{Reason}} 
& \multicolumn{7}{c}{\textbf{Tool-use}} \\
\cmidrule(lr){2-8}\cmidrule(lr){9-15}
& \multicolumn{5}{c}{\textbf{Pass@k}} & \multicolumn{2}{c}{\textbf{Self-choice}} 
& \multicolumn{5}{c}{\textbf{Pass@k}} & \multicolumn{2}{c}{\textbf{Self-choice}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-8}\cmidrule(lr){9-13}\cmidrule(lr){14-15}
& \textbf{p@1} & \textbf{p@2} & \textbf{p@3} & \textbf{p@4} & \textbf{p@8} & \textbf{point-wise} & \textbf{pair-wise}
& \textbf{p@1} & \textbf{p@2} & \textbf{p@3} & \textbf{p@4} & \textbf{p@8} & \textbf{point-wise} & \textbf{pair-wise} \\
\midrule
Qwen3-Next        & -- & -- & -- & -- & -- & -- & --  & 0.57 & 0.64 & 0.70 & 0.73 & -- & 0.42 & -- \\
Qwen3-235B        & -- & -- & -- & -- & -- & -- & --  & 0.52 & 0.60 & 0.63 & 0.65 & -- & -- & -- \\
DeepSeek-V3.2     & -- & -- & -- & -- & -- & -- & --  & 0.59 & 0.69 & 0.71 & 0.75 & -- & -- & -- \\
DeepSeek-R1-0528  & -- & -- & -- & -- & -- & -- & --  & 0.40 & 0.47 & 0.48 & 0.53 & -- & -- & -- \\
Gemini-2.5 Flash  & -- & -- & -- & -- & -- & -- & --  & 0.52 & 0.57 & 0.58 & 0.61 & -- & 0.46 & 0.46 \\
\bottomrule
\end{tabular}
}
\caption{Pass@k and self-choice (point-wise / pair-wise) results across domains under the Omni-agent setting.\cx{the p at k can also be a plot, and self-choice can be a seperate smalle table? I like the side by side pot of two scaling in the previous version} \cx{this table is not very important and acn discard, till rebuttal}}
% \caption{Pass@k and self-choice (point-wise / pair-wise) results across domains under the Omni-agent setting.}
\label{tab:omni_passk_selfchoice}
\end{table*}


==> tables/omni_sequential_scaling.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.9}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l *{2}{c c c c c}}
\toprule
\multirow{2}{*}{\textbf{Omni (Model)}} 
& \multicolumn{5}{c}{\textbf{Search}} 
& \multicolumn{5}{c}{\textbf{Code}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
& \textbf{64k} & \textbf{80k} & \textbf{96k} & \textbf{112k} & \textbf{128k}
& \textbf{64k} & \textbf{80k} & \textbf{96k} & \textbf{112k} & \textbf{128k} \\
\midrule
Qwen3-Next        & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- \\
Qwen3-235B        & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- \\
DeepSeek-V3.2     & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- \\
DeepSeek-R1-0528  & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- \\
Gemini-2.5 Flash  & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- \\
\midrule
\addlinespace[4pt]

\multirow{2}{*}{\textbf{Omni (Model)}} 
& \multicolumn{5}{c}{\textbf{Reason}} 
& \multicolumn{5}{c}{\textbf{Tool-use}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
& \textbf{64k} & \textbf{80k} & \textbf{96k} & \textbf{112k} & \textbf{128k}
& \textbf{64k} & \textbf{80k} & \textbf{96k} & \textbf{112k} & \textbf{128k} \\
\midrule
Qwen3-Next        & -- & -- & -- & -- & --  & 0.62 & 0.54 & 0.41 & 0.40 & 0.40 \\
Qwen3-235B        & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- \\
DeepSeek-V3.2     & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- \\
DeepSeek-R1-0528  & -- & -- & -- & -- & --  & -- & -- & -- & -- & -- \\
Gemini-2.5 Flash  & -- & -- & -- & -- & --  & 0.66 & 0.50 & 0.48 & 0.47 & 0.45 \\
\bottomrule
\end{tabular}
}
\caption{Sequential scaling results across domains under the Omni-agent setting, evaluated at increasing context budgets (64k--128k). \cx{no need}}
% \caption{Sequential scaling results across domains under the Omni-agent setting, evaluated at increasing context budgets (64k--128k).}
\label{tab:omni_sequential_scaling}
\end{table*}

